Fast Commitment for Geo-Distributed Transactions via Decentralized Co-coordinators

In a geo-distributed database, data shards and their respective replicas are deployed in distinct datacenters across multiple regions, enabling regional-level disaster recovery and the ability to serve global users locally. However, transaction processing in geo-distributed databases requires multiple cross-region communications, especially during the commit phase, which can significantly impact system performance. To optimize the performance of geo-distributed transactions, we propose Decentralized Two-phase Commit (D2PC), a new transaction commit protocol aiming to minimize the negative impact of cross-region communication. In D2PC, we employ multiple co-coordinators that perform commit coordination in parallel. Each co-coordinator is responsible for collecting 2PC votes and making a PreCommit decision in its local region. This approach allows for the concurrent invocation of multiple cross-region network round trips, and each region can conclude its concurrency control locally before replication is complete, thus significantly reducing the chances of blocking and enhancing system concurrency. Moreover, we propose the bypass leader replication reply method, leveraging decentralized co-coordinators to bypass the leader for message transmission, thereby reducing the commit latency. Experimental results have demonstrated that D2PC can reduce commit latency by 43% and improve throughput by up to 2.43 times compared to the existing alternative geo-distributed transaction processing methods.

==> design1.tex <==
\subsection{Paralleling 2PC and Replication}\label{design_parallel}
\zzh{Besides the commit latency reduction brought by decentralized commit coordination, we further reduce the commit latency by paralleling 2PC and replication.}

In the layered mode, two essential steps need to be completed before the coordinator can decide to commit: 2PC vote collection (receiving votes from all participants), and replication (where all participant leaders replicate the transaction log and their vote, and the coordinator replicates the commit decision). As illustrated in Fig.~\ref{2pc}, the two steps are interleaved, with Process \ding{192} and \ding{194} are for 2PC, and process \ding{193} and \ding{195} are for replication. The interleaving causes all message delays of 2PC and replication to be included in the waiting time, resulting in high commit latency. However, the processes of 2PC and replication are independent of each other. There is no inherent need for them to wait for one another. If they can run in parallel, the overall commit latency can be reduced.

We intended to \textit{maximize the parallelism of messages.} Firstly, we clarify that the coordination that co-locates with the client is the primary coordinator, which is the arbitrator of the transaction initiated by this client. Message parallelism is reflected in two aspects. ($i$) Upon receiving the \prepare message, the participant leader sends the replication message and 2PC vote in parallel, e.g., message \ding{173} and \ding{174} in Fig.~\ref{overview}(a). ($ii$) As each participant follower receives the replication message, it promptly responds not only to its leader but also to the primary coordinator in parallel, e.g., message \ding{175} in Fig.~\ref{overview}(a). By doing so, the primary coordinator can directly obtain the replication results from followers, eliminating the waiting time typically required to receive the information from leader. 

In these ways, we can separately analyze the delay of 2PC and replication. Referring to Fig.~\ref{overview} (b), for replication, after 1.5 \cross RTTs, the primary coordinator has received the replies from each participant's majority of followers (message \ding{175}), which indicates that replication on each participant shards has been finished. Before that, the primary coordinator has also received all participants' votes (message \ding{173}), so the primary coordinator can safely commit the transaction.


%, and in 3-replica deployment, it only takes 1 RTT to commit a transaction.
% the coordinator decide to commit a transaction when two conditions are satisfied, one is that the votes of all participants are received, the other is that all participant leader has replicated the transaction log and its vote to majority of followers. 



==> design_decentralized_v1.tex <==
\subsection{Changing the Transaction Commit Coordination Pattern}\label{design_decentralized}
%We analyse that the single coordinator will also lead to high commit latency and long transaction critical path. 
%long cc 原因: 1. 单点协调，投票和决定通知引入跨区域通讯；3. 延迟写入可见

%先讲去中心化，然后讲基于去中心化，我们进一步通过两个技术parallel和ewv缩短cc，parallel和ewv都是建立在去中心化之上的


In \gddb database, the location of the coordinator plays a crucial role in determining the \cc length. Specifically, when the coordinator is located in a different region than participant leaders, the communication of the commit decision to them introduces a \cross network delay, as depicted by Process \ding{196} in Fig.~\ref{2pc}. Consequently, this delay results in an extended waiting time for participant leaders to complete the transaction and end the \cc, leading to long \cc.

These drawbacks primarily arise from the reliance on a single coordinator in the 2PC protocol, making the coordinator's location a critical factor. To address this, we propose a modification to the transaction commit coordinator pattern, shifting from centralized commit coordination to decentralized commit coordination. This approach involves deploying a set of coordinators across all datacenters. By doing so, each server can co-locate with a coordinator and be served locally. Therefore, the notification of the commit decision from the coordinator to the participant leader is transferred to intra-datacenter message, which reduces the waiting time for participant leaders. 

Based on the decentralized commit coordination pattern, we further propose two designs to short the \cc length.

%the centralized commit coordination of 2PC plays a crucial role in strength \cc. As only one coordinator can serve, if the coordinator locates in a different region than the participant leaders, the communication between the coordinator and participant leaders will introduce a \cross network delay, as depicted by Process \ding{196} in Fig.~\ref{2pc}. 

% the location of the coordinator plays a crucial role in determining the commit latency and \cc. Specifically, when the coordinator is located in a different region than the client and participant leaders, the communication of the commit result to them introduces a \cross network delay, as depicted by Process \ding{196} in Fig.~\ref{2pc}. Consequently, this delay results in an extended waiting time for the client and participant leaders to complete the transaction and end the \cc, leading to high commit latency and long \cc.

%\hhq{In \gddb databases, the coordinator may not be located in the same region as client and participant leaders, which leads to high commit latency and long \cc. More specifically, when the coordinator and client are located in different regions, the notification of the commit result to the client will introduce one \cross network delay (Process \ding{196} in Fig.~\ref{2pc}). Similarly, for participant leaders that are far away from the coordinator, the messages between them are also \cross (Process \ding{194} and \ding{196}). }
%which is the reason for the long \cc.

%These drawbacks are mainly due to the fact that in the 2PC protocol, there is only one coordinator to serve, causing its location to be a crucial factor. Therefore, we explore changing the transaction commit coordinator pattern, which \textit{turns centralized commit coordination to decentralized commit coordination} by deploying a set of coordinators that are distributed in all datacenters, so that all servers can co-locate with a coordinator and be served locally. In a decentralized way, each coordinator works independently to collect the votes of participants and make the commit decision, then immediately notifies the client and participant leaders in the same datacenter about the decision. This gives the opportunity to short \cc and reduce commit latency.

%In a decentralized manner, each coordinator works independently, gathering participant votes and making commit decisions. Then the coordinator then promptly notifies the client and participant leaders within the same datacenter about the decision. This gives the opportunity to short \cc and reduce commit latency.

\vspace{1mm}

\noindent \textbf{Paralleling the Process of 2PC Voting and Replication.} In the layered mode, two essential steps need to be completed before the coordinator can decide to commit: 2PC vote collection (receiving votes from all participants), and replication (where all participant leaders replicate the transaction log). As illustrated in Fig.~\ref{2pc}, the two steps are serial, with process \ding{192} and \ding{194} for 2PC, and process \ding{193} for replication. The serial of processes causes all message delays replication to be included in the waiting time for participant leaders to receive the commit decision, resulting in long \cc. However, the processes of 2PC and replication are independent of each other. There is no inherent need for 2PC voting to wait until replication is finished. If they can run in parallel, the coordinator can make a \precommit decision early and help shorten the length of \cc.

Based on decentralized commit coordination, we intend to \textit{maximize the parallelism of processes} by allowing leaders directly sends the vote to all coordinators in parallel with replication, without waiting for replication to be finished. In this way, each coordinator can collect votes in advance and immediately notifies the co-located participant leaders about the \precommit decision. However, considering that participant leaders sending the vote to all coordinators may incur extra costs on leaders, we eliminate this effect by merging the vote message and replication message. As depicted in Fig.~\ref{overview}(a), when a participant leader receives the \prepare message, it replicates the transaction log to followers and attaches its vote on the replication message (message \ding{174}), then each follower will send the vote to the co-located coordinator (message \ding{175}). Therefore, each coordinator can collect votes for the co-located replicas after they receive the replication message from the leader. 

In this way, coordinators can make the \precommit decision before the replication is finished, and promptly notify the co-located participant leaders about the decision (message \ding{176}). The early notification of \precommit decision gives participant leaders the opportunity to end \cc early as described following.

%Firstly, we clarify that the coordination that co-locates with the client is the \primary, which is the arbitrator of the transaction initiated by this client. Message parallelism is reflected in two aspects. ($i$) Upon receiving the \prepare message, the participant leader sends the replication message and 2PC vote in parallel, e.g., message \ding{173} and \ding{174} in Fig.~\ref{overview}(a). ($ii$) As each participant follower receives the replication message, it promptly responds not only to its leader but also to the \primary in parallel, e.g., message \ding{175} in Fig.~\ref{overview}(a). By doing so, the \primary can directly obtain the replication results from followers, eliminating the waiting time typically required to receive the information from leader. 

%In these ways, we can separately analyze the delay of 2PC and replication. Referring to Fig.~\ref{overview} (b), for replication, after 1.5 \cross RTTs, the \primary has received the replies from each participant's majority of followers (message \ding{175}), which indicates that replication on each participant shards has been finished. Before that, the \primary has also received all participants' votes (message \ding{173}), so the \primary can safely commit the transaction.
\begin{figure}[t]
	%\vspace{-4mm}
	\centerline{\includegraphics[width=10.3cm]{figure/overview.pdf}}
	\vspace{-2mm}
	\caption{Example of how to shorten the \cc and reduce the commit latency in \ourwork.}
	%\caption{An example of decisions making by \leaderless methods.}
	%\vspace{-5mm}
	\label{overview}
\end{figure}


\vspace{1mm}


\noindent \textbf{Early Write Visibility.} As introduced in \S~\ref{background3}, the database usually delays the write visibility, which results in the \cc to include the network delay of replication.
One way to address this issue is to enable earlier writes visible, allowing \cc to end without waiting for the transaction to be committed. Early write visibility can lead to short \cc and improve transaction processing concurrency, but it may face some challenges. Since early write visibility can potentially compromise the serializability and recoverability, it is necessary to enforce the final commit order to be consistent with the dependency order to ensure correctness \cite{recoverable, swv1, swv2, swv3}. 

%Meanwhile, minimizing the cost of cascading aborts caused by early write visibility. We conclude the aborts may occur in two situations:

%\begin{itemize}
%    \item [1.] deterministic aborts: aborts caused by program logic, such as accessing a non-existent data item; or aborts initiated by the database system, such as those caused by concurrency control and deadlock detection.
%    \item [2.] Non-deterministic aborts: aborts caused by node failures.
%\end{itemize}

By leveraging decentralized commit coordination, participant leaders can obtain the \precommit decision earlier from the co-located coordinator (e.g., message \ding{176} in Fig.~\ref{overview}(a)) instead of waiting for the final \commit message after replication is finished. At this stage, the global serial order of transactions has already been determined, as all participant shards have agreed to commit. Therefore, ending \cc at this point not only excludes the bother of aborts caused by violating serializable, but also can shorten \cc. As illustrated in Fig.~\ref{overview}(a), the shard S$_{1}$'s leader starts \cc when receiving message \ding{172}, and after receiving the vote from shard S$_{2}$, it is aware of the \precommit decision made by the co-located coordinator and ends \cc. Consequently, the length of \cc is only 0.5 \cross RTT. After that, \ourwork will trace \raw dependency to ensure recoverability (details in \S~\ref{shorten_path}).

%\noindent \textbf{Reduce commit latency.} In the decentralized coordination pattern, a coordinator is always co-located with the client, the notification of the commit decision to the client is intra-datacenter (i.e., message \ding{176} in Fig.~\ref{overview}(b)). This eliminates one \cross network delay. Moreover, the presence of multiple coordinators enhances the fault tolerance of the commit decision, eliminating the network latency caused by replicating the commit decision (Process \ding{196} in Fig.~\ref{2pc}). Therefore, the commit latency can be further reduced by 1 \cross RTT.

%Since after the replication of each participant shard is finished, their votes are already stored on more than \majority + 1 servers, therefore, even if the \primary fails, the commit decision can be recovered by running the termination protocol as described in \S~\ref{fault-tolerance}. As a result, the overall commit latency of \ourwork is 1.5 \cross RTTs, and in three-replica deployment, the latency can be reduced to only 1 \cross RTT (details in \S~\ref{fast_commit}).}

%Fig.~\ref{overview} gives an example of how to reduce the commit latency and shorten the \cc with decentralized commit coordination. As the notification from the co-locate coordinator is intra-datacenter (i.e., message \ding{176} in Fig.~\ref{overview}(a) and message \ding{174} in Fig.~\ref{overview}(b)), the commit latency can eliminate one \cross network delay compared to the classical commit approach in Fig.~\ref{2pc}, the participant leader can also be aware of the decision in advance and has the opportunity to end the \cc early (\S~\ref{design_shorten_path}).


%(since each coordinator can only make the decision according to the votes of each participant, they always make the consistent commit decision)

%After that, the participant leaders are aware that the transaction can be committed on all involved shards, which means the serial order is already determined, so it is a safe time to end the \criticalpath which will not violate global serializability. Therefore, the whole \criticalpath can be drastically reduced to 0.5 RTT. 

%Besides, decentralized commit coordination can also reduce the commit latency, as there is always a coordinator in the same datacenter with the client, which is act as the \textit{\primary} to notify the client about the final commit result. As the notification is intra-datacenter (e.g., message \ding{176} in Fig.~\ref{overview}(a)), the commit latency can be reduced by 0.5 \cross RTT compared to the classical commit approach in Fig.~\ref{2pc}.}





%\subsection{Shorten \CC}\label{design_shorten_path}

%As introduced in \S~\ref{background3}, the database usually delays the write visibility causing the \cc to include the network delay of replication, leading to long \cc.
%One way to solve this issue is to make writes visible earlier, i.e., to end concurrency control without waiting for the transaction to be committed. Early write visibility will shorten \cc and improve transaction processing concurrency, but it will also face some challenges. Since early write visibility will break the serializability and recoverability of transactions, it is necessary to force the final commit order to be consistent with the dependency order to ensure correctness \cite{recoverable, swv1, swv2, swv3}. Meanwhile, to minimize the cost of cascading aborts caused by early write visibility, we first conclude the aborts may occur in two situations:

%which in turn will create the problem of cascading aborts \cite{recoverable}, because once a transaction is aborted, all transactions that depend on it will also be aborted. Once a transaction is aborted, all the transactions that depend on it will be aborted as well. Therefore, it is a challenge to choose the right time to reduce the overhead of tracking transaction dependencies and to avoid cascading aborts as much as possible.

%Transaction aborts in databases usually occur in two situations:
%\begin{itemize}
%    \item [1.] deterministic aborts: aborts caused by program logic, such as accessing a non-existent data item; or aborts initiated by the database system, such as those caused by concurrency control and deadlock detection.
%    \item [2.] Non-deterministic aborts: aborts caused by node failures.
%\end{itemize}

%Benefiting from decentralized commit coordination, participant leaders can learn the commit decision from the local coordinator (e.g., message \ding{174} in Fig.~\ref{overview}(b)) earlier than receiving the final \commit message. At this time, the global serial order of transactions has been determined, since all participant shards have agreed to commit. Therefore, end \cc at this time will not only exclude the bother of deterministic aborts, but also can shorten \cc to gain more concurrency. As shown in Fig.~\ref{overview}(b), the leader of shard S$_{1}$ starts \cc when receiving message \ding{172}, and only waiting for the vote from shard S$_{2}$, it can aware of the commit decision from the co-located coordinator and end the \cc, so the length of \cc is only 0.5 \cross RTT. After that, \ourwork will trace \raw dependency to keep the database recoverability (details in \S~\ref{shorten_path}).

%To achieve early write visibility, once \ourwork has received the commit decision from the local coordinator, it will end the \cc (e.g., releasing locks for 2PL and removing the transaction from the validation list for OCC). Then \ourwork will trace RAW dependency to keep the database recoverability (details in \S~\ref{shorten_path}).

%If the \cc ends prematurely, e.g., the leader of each slice ends immediately after this node completes concurrency control, when the global order of transactions has not yet been determined, and if other slices choose to abort the transaction, the slice will eventually abort the transaction as well. Such an abort is deterministic and will result in a large number of cascading rollbacks. If locks are released after the global order has been determined, the transaction will not be affected by deterministic aborts, and given that node failures are infrequent, the probability of a transaction aborting is greatly reduced, avoiding the performance loss associated with massive cascade rollbacks. Moreover, after the global serial order is determined, the serialization can be satisfied, and only the Read After Write (RAW) dependencies need to be tracked for the purpose of ensuring recoverability, and the overhead of transaction dependency tracking will be reduced. Therefore, the plan of this chapter is to enable each participating slice to be informed of the transaction commit decision as early as possible, thus shortening the \cc.



==> design_decentralized_v2.tex <==
\subsection{Changing the Transaction Commit Coordination Pattern}\label{design_decentralized}
%We analyse that the single coordinator will also lead to high commit latency and long transaction critical path. 
%long cc 原因: 1. 单点协调，投票和决定通知引入跨区域通讯；3. 延迟写入可见

%先讲去中心化，然后讲基于去中心化，我们进一步通过两个技术parallel和ewv缩短cc，parallel和ewv都是建立在去中心化之上的


%In \gddb database, 
The location of the coordinator plays a crucial role in determining the \cc length. Specifically, when the coordinator is located in a different region than the participant leader, the communication of the commit decision to them introduces a \cross network delay. Consequently, this delay results in an extended waiting time for participant leaders to complete the transaction and end the \cc, leading to long \cc.

We observe that these drawbacks primarily arise from the reliance on a single coordinator in the 2PC protocol, making the coordinator's location a critical factor. To address this, we propose a modification to the transaction commit coordinator pattern, shifting from centralized commit coordination to decentralized commit coordination. This approach involves deploying a set of coordinators across all datacenters. By doing so, each server can co-locate with a coordinator and be served locally. Therefore, the notification of the commit decision from the coordinator to the participant leader is transferred to intra-datacenter message, which reduces the waiting time for participant leaders. Based on the decentralized commit coordination pattern, we further propose the design to shorten the \cc length.

%the centralized commit coordination of 2PC plays a crucial role in strength \cc. As only one coordinator can serve, if the coordinator locates in a different region than the participant leaders, the communication between the coordinator and participant leaders will introduce a \cross network delay, as depicted by Process \ding{196} in Fig.~\ref{2pc}. 

% the location of the coordinator plays a crucial role in determining the commit latency and \cc. Specifically, when the coordinator is located in a different region than the client and participant leaders, the communication of the commit result to them introduces a \cross network delay, as depicted by Process \ding{196} in Fig.~\ref{2pc}. Consequently, this delay results in an extended waiting time for the client and participant leaders to complete the transaction and end the \cc, leading to high commit latency and long \cc.

%\hhq{In \gddb databases, the coordinator may not be located in the same region as client and participant leaders, which leads to high commit latency and long \cc. More specifically, when the coordinator and client are located in different regions, the notification of the commit result to the client will introduce one \cross network delay (Process \ding{196} in Fig.~\ref{2pc}). Similarly, for participant leaders that are far away from the coordinator, the messages between them are also \cross (Process \ding{194} and \ding{196}). }
%which is the reason for the long \cc.

%These drawbacks are mainly due to the fact that in the 2PC protocol, there is only one coordinator to serve, causing its location to be a crucial factor. Therefore, we explore changing the transaction commit coordinator pattern, which \textit{turns centralized commit coordination to decentralized commit coordination} by deploying a set of coordinators that are distributed in all datacenters, so that all servers can co-locate with a coordinator and be served locally. In a decentralized way, each coordinator works independently to collect the votes of participants and make the commit decision, then immediately notifies the client and participant leaders in the same datacenter about the decision. This gives the opportunity to short \cc and reduce commit latency.

%In a decentralized manner, each coordinator works independently, gathering participant votes and making commit decisions. Then the coordinator then promptly notifies the client and participant leaders within the same datacenter about the decision. This gives the opportunity to short \cc and reduce commit latency.

%\vspace{1mm}

% 原本流程里两者是interleaving的，我们观察到可以将两者分离并且并行起来，这样vote能够先于replication，从而给了缩短cc的机会。具体来说（讲一下流程），然后再结合ewv


%\noindent \textbf{Paralleling the Process of 2PC Voting and Replication.}
In the layered mode, two essential steps need to be completed before the coordinator can decide to commit: 2PC vote collection (receiving votes from all participants), and replication (where all participant leaders replicate the transaction log). As illustrated in Fig.~\ref{2pc}, the two steps are interleaving, with process \ding{192} and \ding{194} for 2PC, and process \ding{193} for replication. The interleaving of processes causes all message delays to be included in the waiting time for participant leaders to receive the commit decision.

However, we observe that the processes of 2PC and replication are independent of each other, if they can run in parallel, the vote collection can be finished before the replication (as shown in Fig.~\ref{overview}, the second dashed red line can be regarded as the time of finishing vote collection, and the third dashed red line is the time of finishing replication). Therefore, we intend to \textit{decouple the processes of 2PC and replication.} Based on decentralized commit coordination, \emph{each coordinator can collect votes and make a \precommit decision early}, which helps shorten the length of \cc.

Decoupling 2PC and replication makes that we can optimize the \cc length and commit latency independently.
Therefore, in Fig.~\ref{overview}, (a) shows the reduction in \cc length, and (b) shows the optimization of commit latency (\S~\ref{design_bypass leader}). 

Specifically, by allowing leaders directly sends the vote to all coordinators in parallel with replication, each coordinator can collect votes in advance and immediately notifies the co-located participant leaders about the \precommit decision. However, considering that participant leaders sending the vote to all coordinators may incur extra costs on leaders, we eliminate this effect by merging the vote message and replication message. As depicted in Fig.~\ref{overview}(a), when a participant leader receives the \prepare message, it replicates the transaction log to followers and attaches its vote on the replication message (message \ding{173}), then each follower will send the vote to the co-located coordinator, e.g., the follower of S$_{1}$ and S$_{3}$ sends the vote to the co-located coordinator in DC$_{2}$ once they receive the replication message from their leader. 

\begin{figure*}[t]
	%\vspace{-4mm}
	\centerline{\includegraphics[width=19cm]{figure/overview.pdf}}
	\vspace{-2mm}
	\caption{Example of how to shorten the \cc and reduce the commit latency in \ourwork.}
	%\caption{An example of decisions making by \leaderless methods.}
	%\vspace{-5mm}
	\label{overview}
\end{figure*}

After the coordinator collects votes from the co-located replicas (message \ding{174}), it can make the \precommit decision before the replication is finished, and promptly notify the co-located participant leaders about the decision (message \ding{175}). The notification of \precommit decision gives participant leaders the opportunity to end \cc early by \textit{enabling earlier writes visible. }
%\noindent \textbf{Early Write Visibility.} As introduced in \S~\ref{background3}, the database usually delays the write visibility, which results in the \cc to include the network delay of replication.
%One way to address this issue is to enable earlier writes visible, allowing \cc to end without waiting for the transaction to be committed. Early write visibility can lead to short \cc and improve transaction processing concurrency, but it may face some challenges. Since early write visibility can potentially compromise the serializability and recoverability, it is necessary to enforce the final commit order to be consistent with the dependency order to ensure correctness \cite{recoverable, swv1, swv2, swv3}. 

%Meanwhile, minimizing the cost of cascading aborts caused by early write visibility. We conclude the aborts may occur in two situations:

%\begin{itemize}
%    \item [1.] deterministic aborts: aborts caused by program logic, such as accessing a non-existent data item; or aborts initiated by the database system, such as those caused by concurrency control and deadlock detection.
%    \item [2.] Non-deterministic aborts: aborts caused by node failures.
%\end{itemize}

By leveraging decentralized commit coordination, participant leaders can obtain the \precommit decision earlier from the co-located coordinator instead of waiting for the final \commit message after replication is finished. At this stage, the global serial order of transactions has already been determined, as all participant shards have agreed to commit. Therefore, ending \cc at this point not only excludes the bother of aborts caused by violating serializable, but also can shorten \cc. As illustrated in Fig.~\ref{overview}(a), the each shard leader starts \cc when receiving message \ding{172}, and after receiving the \precommit decision made by the co-located coordinator and ends \cc. Consequently, the length of \cc is only 0.5 \cross RTT, which is significantly shorter than the \cc length of \layered and \integrate as described in \S~\ref{background2}. 
%After that, \ourwork will trace \raw dependency to ensure recoverability (details in \S~\ref{shorten_path}).

%\noindent \textbf{Reduce commit latency.} In the decentralized coordination pattern, a coordinator is always co-located with the client, the notification of the commit decision to the client is intra-datacenter (i.e., message \ding{176} in Fig.~\ref{overview}(b)). This eliminates one \cross network delay. Moreover, the presence of multiple coordinators enhances the fault tolerance of the commit decision, eliminating the network latency caused by replicating the commit decision (Process \ding{196} in Fig.~\ref{2pc}). Therefore, the commit latency can be further reduced by 1 \cross RTT.

%Since after the replication of each participant shard is finished, their votes are already stored on more than \majority + 1 servers, therefore, even if the \primary fails, the commit decision can be recovered by running the termination protocol as described in \S~\ref{fault-tolerance}. As a result, the overall commit latency of \ourwork is 1.5 \cross RTTs, and in three-replica deployment, the latency can be reduced to only 1 \cross RTT (details in \S~\ref{fast_commit}).}

%Fig.~\ref{overview} gives an example of how to reduce the commit latency and shorten the \cc with decentralized commit coordination. As the notification from the co-locate coordinator is intra-datacenter (i.e., message \ding{176} in Fig.~\ref{overview}(a) and message \ding{174} in Fig.~\ref{overview}(b)), the commit latency can eliminate one \cross network delay compared to the classical commit approach in Fig.~\ref{2pc}, the participant leader can also be aware of the decision in advance and has the opportunity to end the \cc early (\S~\ref{design_shorten_path}).


%(since each coordinator can only make the decision according to the votes of each participant, they always make the consistent commit decision)

%After that, the participant leaders are aware that the transaction can be committed on all involved shards, which means the serial order is already determined, so it is a safe time to end the \criticalpath which will not violate global serializability. Therefore, the whole \criticalpath can be drastically reduced to 0.5 RTT. 

%Besides, decentralized commit coordination can also reduce the commit latency, as there is always a coordinator in the same datacenter with the client, which is act as the \textit{\primary} to notify the client about the final commit result. As the notification is intra-datacenter (e.g., message \ding{176} in Fig.~\ref{overview}(a)), the commit latency can be reduced by 0.5 \cross RTT compared to the classical commit approach in Fig.~\ref{2pc}.}





%\subsection{Shorten \CC}\label{design_shorten_path}

%As introduced in \S~\ref{background3}, the database usually delays the write visibility causing the \cc to include the network delay of replication, leading to long \cc.
%One way to solve this issue is to make writes visible earlier, i.e., to end concurrency control without waiting for the transaction to be committed. Early write visibility will shorten \cc and improve transaction processing concurrency, but it will also face some challenges. Since early write visibility will break the serializability and recoverability of transactions, it is necessary to force the final commit order to be consistent with the dependency order to ensure correctness \cite{recoverable, swv1, swv2, swv3}. Meanwhile, to minimize the cost of cascading aborts caused by early write visibility, we first conclude the aborts may occur in two situations:

%which in turn will create the problem of cascading aborts \cite{recoverable}, because once a transaction is aborted, all transactions that depend on it will also be aborted. Once a transaction is aborted, all the transactions that depend on it will be aborted as well. Therefore, it is a challenge to choose the right time to reduce the overhead of tracking transaction dependencies and to avoid cascading aborts as much as possible.

%Transaction aborts in databases usually occur in two situations:
%\begin{itemize}
%    \item [1.] deterministic aborts: aborts caused by program logic, such as accessing a non-existent data item; or aborts initiated by the database system, such as those caused by concurrency control and deadlock detection.
%    \item [2.] Non-deterministic aborts: aborts caused by node failures.
%\end{itemize}

%Benefiting from decentralized commit coordination, participant leaders can learn the commit decision from the local coordinator (e.g., message \ding{174} in Fig.~\ref{overview}(b)) earlier than receiving the final \commit message. At this time, the global serial order of transactions has been determined, since all participant shards have agreed to commit. Therefore, end \cc at this time will not only exclude the bother of deterministic aborts, but also can shorten \cc to gain more concurrency. As shown in Fig.~\ref{overview}(b), the leader of shard S$_{1}$ starts \cc when receiving message \ding{172}, and only waiting for the vote from shard S$_{2}$, it can aware of the commit decision from the co-located coordinator and end the \cc, so the length of \cc is only 0.5 \cross RTT. After that, \ourwork will trace \raw dependency to keep the database recoverability (details in \S~\ref{shorten_path}).

%To achieve early write visibility, once \ourwork has received the commit decision from the local coordinator, it will end the \cc (e.g., releasing locks for 2PL and removing the transaction from the validation list for OCC). Then \ourwork will trace RAW dependency to keep the database recoverability (details in \S~\ref{shorten_path}).

%If the \cc ends prematurely, e.g., the leader of each slice ends immediately after this node completes concurrency control, when the global order of transactions has not yet been determined, and if other slices choose to abort the transaction, the slice will eventually abort the transaction as well. Such an abort is deterministic and will result in a large number of cascading rollbacks. If locks are released after the global order has been determined, the transaction will not be affected by deterministic aborts, and given that node failures are infrequent, the probability of a transaction aborting is greatly reduced, avoiding the performance loss associated with massive cascade rollbacks. Moreover, after the global serial order is determined, the serialization can be satisfied, and only the Read After Write (RAW) dependencies need to be tracked for the purpose of ensuring recoverability, and the overhead of transaction dependency tracking will be reduced. Therefore, the plan of this chapter is to enable each participating slice to be informed of the transaction commit decision as early as possible, thus shortening the \cc.



==> response.tex <==
% % 添加两个环境变量
% \newenvironment{tablehere}
% {\def\@captype{table}}

% \newenvironment{figurehere}
% {\def\@captype{figure}}


\section*{Responses to Reviewer \#1}
~\
% 论文中相应要改动的：1. 关于并发控制周期的描述，分开讨论OCC和2PL。2. 再总结下novelty，不是简单的ELR在分布式事务中应用，而是设计了decentralized提交协调，从而有了ELR的机会。


\textbf{O1:} Even though the paper claims that D2PC applies to both 2PL and OCC, it actually assumes OCC. Unless this reviewer misunderstands, if one wants to achieve fairness and starvation-freeness on top of it, locking time will be almost the same as 2PL. 

\response Starvation is indeed possible in our origin protocol. As described in Section 4.5, D2PC allows reading data from local replicas to reduce read latency. When combined with 2PL, this eliminates the necessity of read locks during execution. This optimization is also adopted in Carousel\cite{carousel}. As the example given by Reviewer 1 shows, if a transaction performs read without acquiring read locks, the read items can be updated by other transactions, forcing the read transaction to abort due to reading stale data. This may occur repeatedly, resulting in starvation.

To illustrate this issue, we altered the Retwis workload, making each read-only transaction read 50 keys, and set the proportion of read-only transactions to 50\%. %Without the acquisition of read locks during execution, long read transactions can be susceptible to repeated aborts, leading to starvation. 
As shown in the following table, a significant proportion of the read-only transactions are susceptible to starvation, due to repeated aborts.
In the table, \dlocks represents our origin protocol that adopts local read optimization but lacks a starvation solution, and \ourworknro represents the \ourwork variant without adopting the read optimization, which means that it acquires read lock upon each read. We measured transaction retry times, designating transactions with more than five retries as starved transactions. The results indicate that \dlocks suffers from starvation, whereas \ourworknro does not.
It is worth noting that, to avoid excessive remote reads, we adopted the one-shot transactions mode used in ~\cite{carousel}, making sure that the reads of each transaction occur in a single round.

\begin{table}[H]
	\centering
	%\vspace{-4mm}
	\caption*{\bf Table. Proportion of starved transactions under different client numbers.}
	\vspace{-2mm}
 %\resizebox{\textwidth}{15mm}{
 \resizebox{0.9\columnwidth}{!}{
	\begin{tabular}{c|ccccc}
		%\toprule[1pt]
		\textbf{\makecell[c]{Client Number}} & \textbf{30} & \textbf{60} & \textbf{90} & \textbf{120} & \textbf{150} \\
		%\midrule
		\hline
		\textbf{\dlocks} & 5.2\% & 7.3\% &  10.1\% & 13.9\% & 17.6\%\\
		\textbf{\ourworknro} & 0\% & 0\% & 0\% & 0\% & 0\%\\
        \textbf{\dlocksf} & 0\% & 0\% & 0\% & 0\% & 0\%\\
		%\bottomrule[1pt]
		\vspace{-4mm}
	\end{tabular}
 }
\end{table}




% \reminder{Performance:Locking time will be almost the same as 2PL.  D2PC+2PL Performance.}

To address the starvation issue, \ourwork can force each aborted transaction to acquire read locks on the shard leaders during its second round of execution. 
This method ensures transaction latency under non-starvation cases. At the same time, it eliminates starvation when aborts occur. We name this method as \dlocksf. The experiment results in the Table demonstrate its effectiveness in eliminating starvation. 

\begin{figure}[H]
	%\vspace{-2mm}
 
	\centerline{\includegraphics[width=5.5cm]{figure/revise/starvation.pdf}}
 %\vspace{-4mm}
  \caption*{\bf Figure. Throughput with/without read optimization and starvation solution.}  
	%\vspace{-2mm}
	%\vspace{-2mm}
\end{figure}

% 把figure分开写
We conducted a comprehensive throughput evaluation of \dlock, \lock, and \dlocksf. %with and without read optimization and starvation solution, and t
The results are depicted in the Figure above. %We have several observations.

In the figure, both \ourworknro and \locknro disabled read optimization, allowing us to clearly observe the enhancements introduced by \ourwork. We can see that \ourworknro achieves a 1.55~$\times$ increase in throughput compared to \locknro. After the adoption of read optimization, represented by \dlocks and \locks, both approaches achieved significant improvement in throughput. Notably, \dlocks still outperforms \locks, by 1.89 $\times$ in throughput. This means that, whether or not read optimization is employed, \ourwork can consistently enhance performance. Furthermore, the line of \dlocksf illustrates the effectiveness of the aforementioned starvation prevention solution. \dlocksf achieved a slightly higher throughput than \dlocks, due to its ability to prevent starvation.

Besides the experiments under the altered workload, we also conducted experiments to compare \ourworknro against \locknro using the standard Retwis workload. The results are presented in Fig.~\ref{2pl clients}, which demonstrate that \ourworknro is capable of shortening the locking duration by 44\%, 
%when compared to \locknro even when read locks are acquired during execution, enabling \ourworknro to achieve a 
resulting in a significant improvement in throughput. This clearly shows the benefit of \ourwork.


% 4.5加了情况描述，5.2加了读负载实验，我们还比较了标准2pl。解释下5.2节加了哪些
In the revised paper, we discuss the starvation issue and its solution in \S~\ref{optimization}. We also present an additional experimental study under long read transactions in \S~\ref{scalability}, to show the effectiveness of our starvation prevention solution. Moreover, in Fig.~\ref{2pl clients}, we added the comparison of \dlock and \lock, both of which disabled the read optimization, to clearly demonstrate the benefit of \ourwork.
%add some evaluation results in \S~\ref{scalability}.}


%We'll incorporate this starvation solution in the revised paper. while D2PC+2PL and D2PC Starvation-Free will not cause starvation. 
%To achieve fairness and starvation-free, transactions that abort due to stale reads will be forced to require read locks on leader during their second execution. We'll incorporate this starvation solution in the revised paper.

\linespread{1.2}

% \begin{tablehere}
% 	\centering
% 	% \vspace{-1mm}
% 	% \caption{\bf Proportion of starvation transactions under different client numbers.}
% 	% \vspace{-2mm}
%  %\resizebox{\textwidth}{15mm}{
%  \resizebox{0.5\columnwidth}{!}{
% 	\begin{tabular}{c|ccccc}
% 		%\toprule[1pt]
% 		\textbf{\makecell[c]{Client Number}} & \textbf{30} & \textbf{60} & \textbf{90} & \textbf{120} & \textbf{150} \\
% 		%\midrule
% 		\hline
% 		\textbf{\ourwork} & 5.2\% & 7.3\% &  10.1\% & 13.9\% & 17.6\%\\
% 		\textbf{D2PC+2PL} & \hhq{0\%} & 0 & 0 & \hhq{5} & 0\\
%         \textbf{D2PC Starvation-Free} & 0 & 0 & 0 & 0 & 0\\
% 		%\bottomrule[1pt]
% 		\vspace{-2mm}
% 	\end{tabular}
%  }
% \end{tablehere}

% \begin{figurehere}
% 	%\vspace{-4mm}
% 	\centerline{\includegraphics[width=8cm]{figure/revise/starvation.pdf}}
% % \begin{table}
% %     \centering
% %     \caption{\bf Proportion of starvation transactions under different client numbers.}
% % \end{table}
% 	\vspace{-2mm}
% 	\vspace{-5mm}
% \end{figurehere}

% \begin{table}[H]
% 	\centering
% 	% \vspace{-1mm}
% 	\caption{\bf Proportion of starvation transactions under different client numbers.}
% 	\vspace{-15mm}
% \end{table}




\vspace{3mm}


\textbf{O2:} Experiments don’t cover fairness/starvation-freeness and a workload where it’d be clearly exhibited.

\response We conducted an additional set of experiments using a long-read transaction workload, which are more susceptible to starvation, in the evaluation. A detailed analysis of the results is provided in the response to O1 and \S~\ref{scalability}.
% 我们加了相应workload，
%\reminder{O2 only talks about read heavy workload, not about the common case. \response As explained in the response of O1, we modified the workload to demonstrate the starvation. And we set both \dlock and \lock disable read optimization, denoted as \ourworknro and \locknro to clearly show the improvement brought by \ourwork. We can see that when both D2PC and 2PC acquire locks during execution, \ourworknro achieves 1.53 $\times$ throughput than \locknro. 

%The results in Fig~\ref{2pl clients} of \S~\ref{scalability} also show that \ourwork can reduce the transaction latency and locking time when disabling read optimization. The results clearly demonstrate the benefit of \ourwork.}

%\reminder{We add the evaluation of our starvation solution and a clear benefit of \ourwork in \S~\ref{scalability}.}

% In such a workload, 2PC+2PL represents the commit protocol which combines 2PC and 2PL. The results show that when both D2PC and 2PC acquire locks during execution, the throughput of D2PC still achieves 1.53$\times$ than 2PC (D2PC+2PL and 2PC+2PL in figure), and D2PC can reduce the transaction latency by 22\% than 2PC. \reminder{This is because:}This clearly shows the benefit of D2PC when combined with 2PL. 



%\reminder{Normal Cases: D2PC+2PL vs 2PC+2PL}

%After solving the starvation problem, D2PC Starvation-Free can preclude starvation and achieve much higher throughput than 2PC+2PL, which is 3.63 times in throughput and 59\% reduction in latency.
%In our implementation, all methods adopt the read optimization described above. If the starvation solution is integrated, the locking time of all methods will increase when transaction aborts due to stale read, but D2PC still retains the shortest locking time since it can release lock early. In standard scenarios where transactions pass the read version validation, D2PC's advantage is significant. We will update the evaluation once we incorporate the starvation solution.

%\reminder{Modification in the paper.}

\vspace{3mm}
% 强调commit阶段的cc缩减，introduction也要提
\textbf{O3:} Commit latency does not change significantly. Not enough to justify more location-tracking etc in follower-replicas and clients.

\response The primary goal of D2PC is to shorten the concurrency control period during the transaction commit stage to mitigate conflict effects. Reducing commit latency is not our main claim, but D2PC does optimize latency as well. Notably, latency reduction made by D2PC is more significant when the degree of contention is high, as shown in Fig.\ref{2pl clients}, \ref{occ clients}, and \ref{replicas}. %, where it outperforms all methods. 

\vspace{3mm}
% novelty再强调下，以及elr和本文工作的区别
\textbf{O4:} This paper is essentially early-write-visibility applied to distributed transactions. I’m not sure if it’s a substantially new idea or not.

\response Early-write-visibility for distributed transactions has been explored in a number of works, such as DLV~\cite{dlv}. What sets our approach apart is its utilization of decentralized transaction commitment. Decentralizing the coordinator in 2PC yields several benefits. Firstly, decentralized commit coordination permits each datacenter to make a \precommit decision on its own \co, thus giving an opportunity to perform early-write-visibility to enhance scalability. Secondly, leveraging decentralized \co to route replication replies directly to the \primary, bypassing the leader, can reduce transaction latency. Thirdly, decentralized \co can enhance the fault tolerance of the coordinator, simplifying commit decision restoration.

% Decentralized commit coordination permits each datacenter to make a \precommit decision on its own \co, thus giving an opportunity to perform early-write-visibility to enhance scalability. Besides, decentralizing the coordinator also enhances the fault tolerance of the coordinator, and also reduces the transaction latency.


~\\
\vspace{-5mm}
\section*{Responses to Reviewer \#2}
~\
% 相关文献中加多主事务处理
% 再提一下我们的novelty在哪
\textbf{O1:} The paper does not compare to systems based on multi-master replication architecture that also has similar goals as proposed in this paper. For instance, GeoGauss: Strongly Consistent and Light-Coordinated OLTP for Geo-Replicated SQL Database, ACM Manag. Data 2023

\response Multi-master replication aims for scalability by distributing transaction processing across all replicas, without a leader node. In contrast, D2PC chooses to decentralize the coordinator rather than the leader, maintaining a leader-based transaction processing model that is common in practice. Therefore, these two works differ significantly in architectures and transaction models. These differences drive GeoGauss and \ourwork focus on different research aspects. GeoGuss primarily focuses on how to handle inter-node write-write conflicts, while \ourwork aims to decentralize the 2PC protocol to attain the shortest \cc and minimize latency.

Therefore, given the disparate architectures and research aspects in the two works, direct comparisons in the evaluation are not feasible. However, in our related work section (\S~\ref{background2}), we discussed GeoGauss and elaborated the difference between them.

% decentralize the transaction commit coordination to short the \cc and reduce latency, without modification 

%this causes a challenge in handling inter-node write-write conflicts effectively. Therefore, the main contribution of GeoGauss is its coordination-free conflict resolution mechanism. 

%The leader-based transaction processing and decentralized commit coordination enables \ourwork achieve efficient conflict resolution, and also performs well in th
%enabling centralized conflict resolution to minimize aborts. Therefore, D2PC achieves reduced latency and enhanced write scalability while maintaining efficient conflict resolution. We’ll elaborate on the differences with multi-master replication in revised paper. \reminder{Global Time. Better If we claim the two method have different focuses. e.g. they do not have the 2PC phase?}

%  and \reminder{cannot achieve strong consistency.} I

\vspace{3mm}

\textbf{O2:} The evaluation does not evaluate and compare the performance under fault tolerance support.

\response We conducted an additional experiment to evaluate the robustness of \ourwork under \co failures. The result is shown in Fig.~\ref{failure}. While running \ourwork, we artificially shut down two \co servers, to see the impact on performance. The result shows that \ourwork can tolerate \co failures, while the throughput may drop when \co fails. This is mainly because some transactions fail to be precommitted and thus delay the \cc period. Nevertheless, even when there is only one \co alive, \ourwork still outperforms \occ. The results of the evaluation are presented in Section~\ref{scalability}.

\vspace{3mm}

\textbf{-} Clarify the novelty of the work, in particular in combining early write visibility with decentralized commit coordination.

\response The novelty of the work lies in the adoption of decentralized transaction commitment. Decentralizing the coordinator in 2PC yields several benefits. Firstly, decentralized commit coordination permits each datacenter to make a \precommit decision on its own \co, thus giving an opportunity to perform early-write-visibility to enhance scalability. Secondly, leveraging decentralized \co to route replication replies directly to the \primary, bypassing the leader, can reduce transaction latency. Thirdly, decentralized \co can enhance the fault tolerance of the coordinator, simplifying commit decision restoration.







~\\
\vspace{-10mm}
\section*{Responses to Reviewer \#4}
~\

% 在design overview 里加上一个关于事务状态转换的总结
\textbf{O1:} The paper organization and exposition can be greatly improved. Consider making earlier explanations higher level instead of just referencing things that will be explained later. For example consider adding a state diagram showing that a transaction can both abort or commit after pre-commit and specifying what are the conditions needed for a co-coordinator to issue a PreCommit message.

\response Thanks for the suggestions. We have added a transaction state transition graph to the paper, as shown in Fig.~\ref{transition}. A new subsection, \S~\ref{state transition}, was added to describe the conditions of the \precommit state and how a \precommit transaction can be committed or aborted.

\vspace{3mm}

\textbf{O2:} Comparison with related work can be greatly improved. Both in text but also in the evaluation - 2 of the 3 alternatives being compared against in the evaluation section are "layered", but it isn't clear which systems they represent or how realistic they are.

% 我们在图一也明确了
\response The 2PC+2PL is an implementation of Spanner's \cite{spanner1} transaction protocol, while 2PC+OCC can be seen as a variant of Spanner, which adopts OCC as the concurrency control protocol. Similar approaches have been utilized by TAPIR \cite{tapir} and Janus \cite{janus} in their evaluations. We clarified these in Fig~\ref{2pc} and Section~\ref{setup}.

% \reminder{Related Work}

\vspace{3mm}

\textbf{O3:} a local PreCommit decision can be made if information is available from all shards involved in a transaction. It isn't clear how common it is in reality that every datacenter has a replica from all involved shards (of course this only works when the replicas aren't faulty). The evaluation doesn't distinguish between the "fast" path, when this is true, and the "slow" path.

\response Full replication at every datacenter is not mandatory. When the leader sends a replication message, in cases where a datacenter lacks a replica, the leader directly sends its vote to the co-coordinator of that datacenter, Which in turn can still make the \precommit decision.  We emphasized this in Section~\ref{fast_commit}.

Besides, we also conducted an evaluation on the impact of \co failures in Section~\ref{scalability}. The results are shown in Fig.~\ref{failure}. It included the case where two \coss fail simultaneously. In such a case, the transaction cannot be committed on the fast path. In Fig.~\ref{failure}, we can see the performance gap between the fast and slow paths.

%\reminder{the problem of fast path and slow path}

\vspace{3mm}

\textbf{O4:} The mechanics of how a local co-coordinator knows which shards are involved in a given transaction are also not explained. Since the local co-coordinator gets its information from replication, would the shard list need to be included in replication messages ? Similarly, how does the corresponding co-coordinator know which shards are involved in a transaction ? and how does it know to notify the client - do all clients maintain connections to their local co-ordinator ? this seems problematic and unclear why it wouldn't affect performance.

\response In our implementation, each replication message contains the list of the involved shards. We have clarified this in Section~\ref{fast_commit}. We anticipate that this will exert a negligible impact on performance. Considering that TCP/IP packet headers already occupy 40 bytes and a shard ID can be represented in 4 bytes (unit32\_t), the extra bandwidth consumed by transmitting the shard list is small. Moreover, in distributed transactions, the number of involved shards is typically limited, which further mitigates the potential performance consequences.

In our implementation, the client is not directly connected to \co. It only interacts with shard replicas. When a participant shard leader, co-located with the client, receives the commit decision from \primary, it will notify the client about the decision.

 
\vspace{3mm}
% 要在论文里某个地方讲coordinator sharding策略。
\textbf{O5:} The evaluation didn't convince me that the approach is scalable. Now the co-coordinator in its DC is involved in all transactions in the DC. As we add more shards and servers in each data-center, how does having a single co-coordinator per DC scale compared to other approaches ? What about the performance impact of co-coordinator failure ?

\response In our experiments, when we increased the load, we did not see the co-coordinator appear as a bottleneck. As shown in Fig.~\ref{2pl clients} and \ref{occ clients}, when the performance of other methods stabilized, D2PC's performance continued to increase. To verify whether the co-coordinator can become the bottleneck, we ran an additional experiment by equipping the co-coordinator server with only 1 CPU and 512 MB memory, and the result was added to Section~\ref{scalability of co}. As shown in Fig.~\ref{coor_scale}, with limited resources, a co-coordinator could indeed become a bottleneck.
%, as the client number reached 360 when only one \co group was deployed.

To address this problem, we designed a coordinator sharding strategy. In particular, when co-coordinators become overloaded, we can partition them into N groups, with N co-coordinators in each datacenter. In this way, the load of one co-coordinator can be distribute on N co-coordinators by taking the transaction ID modulo N. In Fig.~\ref{coor_scale}, the line of "shared coordinator" represents the performance with N=2, which means there are two co-coordinators per datacenter. As observed, the throughput continues to increase even when the throughput of the individual coordinator group stabilizes. 
Therefore, the experiments show that coordinator sharding is effective in improving the scalability of co-coordinators. We include a detailed explanation of the \co sharding strategy in Section~\ref{shorten_path}, and present the evaluation about the \co scalability in Section~\ref{scalability of co}.

To evaluate the impact of \co failure, we conducted an additional set of experiments. As shown in Fig.~\ref{failure} in Section~\ref{scalability}, while running \ourwork, we artificially shut down two \co servers, and see how it influences the performance. The result shows that \ourwork can tolerate \co failures. The throughput may drop when a \co fails, because some transactions may fail to be precommitted and delay the \cc period. Nevertheless, even when there is only one \co alive, \docc still outperforms \occ. 

\vspace{3mm}

\textbf{Minor remarks:}
~\

\textbf{-} “However, such a layered architecture has to bear the cost of multiple rounds of cross-region communication.” CockroachDB, for example, employs a number of optimizations, such as parallel commits, pipelined transactions, and 1-phase-commit that minimize the number of round-trips. Specifically, with Parallel commits (https://www.cockroachlabs.com/blog/parallel-commits/), instead of waiting for two synchronous round-trips of distributed consensus (prepare, commit) before acknowledging a transaction commit, CockroachDB only waits for one. The location of the transaction coordinator (which is usually local to the client) of course also plays a role and may add to latency. Without further details the claims of “surpassing the performance of state-of-the-art approaches” based just on the number of round-trips seem unjustified (the paper also doesn’t compare performance directly with CockroachDB / TiDB / Spanner).
  
\response In database systems that adopt layered architectures, such as CockroachDB, optimizations such as parallel commits can be used to reduce the commit phase latency of 2PC. %resulting in a single-round consensus commit latency. 
However, this optimization requires that the coordinator and shard leaders are co-located. When shard leaders are geo-distributed, the effectiveness of such optimization is limited. We reviewed this specific optimization adopted by CockroachDB and discussed its limitations in Section~\ref{background2}. 
%providing a detailed explanation rather than a generalized description.

%We introduce the optimization of CockroachDB and its limitation in Section~\ref{background2}, instead of a generalized description.

\vspace{3mm}

\textbf{-} Consider citing E3PC (https://iditkeidar.com/wp-content/uploads/files/ftp/pods-95.pdf) in Section 2.1. It solves some of the issues with 2PC and 3PC and precedes Paxos commit.

\response Thanks for the suggestion. We have cited and briefly discussed E3PC in the related work (Section~\ref{background1}).

\vspace{3mm}

\textbf{-} The example execution of Figure 1 seems similar to Spanner. If so, you should point it out. It doesn’t necessarily represent every layered system.  In particular, its not so clear what a “client” is, and having the client talk directly to shard leaders implies that it has up-to-date knowledge of sharding and leader locations. All the examples in the paper are for this setting, does your approach extend to systems where the client accesses any local server and that server coordinates the request?

\response Yes. Fig. 1 depicts the transaction committing protocol in Spanner. This is clarified in the caption of Fig.~\ref{2pc}. 

In this paper, "client" refers to the application server within the datacenter. It will interact with database servers through the client library described in \S~\ref{design_architecture}. The client library has up-to-date leader locations, and the clients can directly communicate with shard leaders. This is also an assumption of protocols like TAPIR~\cite{tapir} and Carousel~\cite{carousel}.
 
\vspace{3mm}

\textbf{-} In Figure 1 the leaders of the two shards are not in the same data center. Often, if the data is accessed together, they would be Co-located, eliminating the first WAN message (unless the client isn't in the same location).

\response In practice, shard leaders might be located in the same datacenter,  depending on the business logic. However, this arrangement isn't always fixed, and cross-region data access still exists. Our approach is designed for this general scenario. This is aligned with the models in Spanner~\cite{spanner1,spanner2}, Tapir~\cite{tapir}, Janus~\cite{janus}, and Carousel~\cite{carousel}, where participant leaders are geo-distributed. 

\vspace{3mm}
% 改图二
\textbf{-} Figure 2 is referred in the text without being really explained. The explanation appears in later paragraphs of Sec 3.1. Consider reordering the text. The label of figures (a) and (b) doesn’t help unfortunately. Is it possible to make the same point with one instead of two different placement scenarios? Also, for some reason in figure 2(a) the client isn’t in one of the datacenters but in figure 2(b) it is. Can you be consistent about that ? In figure 2(a), where does the concurrency period start and end?

\response Firstly, we refined the description of Fig.~\ref{overview} in Section~\ref{design_decentralized} and \ref{design_bypass leader}. The separation of Figure (a) and (b) is due to the fact that while a single protocol is intended to simultaneously reduce \cc and latency, the processes required to achieve these two effects involve different servers. To enhance clarity in our presentation, we have depicted these scenarios in two distinct figures.

Secondly, we updated Fig.~\ref{overview} to set the client of figure (a) in DC1, which is consistent with figure (b). 

Finally, in Fig.~\ref{overview}(a), the \cc starts and ends on participant leaders. Leaders start \cc when receive the \prepare message, and end \cc when receive the \precommit decision from the co-located \co.

\vspace{3mm}


\textbf{-} What happens if not all shards have a replica in every data center? Or some of these replicas are faulty? For example, if S3 follower in DC2 is offline (assuming there are other replicas elsewhere). It is possible that no single co-coordinator knows whether all shards have agreed to commit. How can writes be made visible only based on local coordinator knowledge? You explain this much later in the paper, it would be helpful to mention it earlier, and perhaps state the PreCommit condition more precisely.

\response If not all shards have replicas in every datacenter, the leader will directly send its vote to the co-coordinator of the datacenter that lacks a replica. We have elaborated this in Section~\ref{fast_commit}.

If a replica fails, the co-located co-coordinator will be unable to make write visible earlier, and the writes will be visible after the final Commit decision is received.

In terms of the condition of \precommit, we have included a transition graph of the transaction state in Fig.~\ref{transition}, and provided detailed explanations about the conditions for the transitions in Section~\ref{state transition}.
 
\vspace{3mm}

\textbf{-} Lines 685-695: “An important observation to highlight is that in the commonly adopted three-replica deployment, the commit latency is only 1 inter-datacenter RTT.” This assumes that the second replica is indeed co-located with the corresponding coordinator. But the number of datacenters might be much bigger than the replication factor of a single item.

\response Only when a replica co-locates with the correspondent coordinator, is the latency 1 \cross RTT. We have clarified it in Section~\ref{fast_commit}.
 
\vspace{3mm}

\textbf{-} Lines 789 - 798: a transaction can abort after pre-committing? That wasn’t clear so far, can you explain how that can happen? I thought that the PreCommit decision is made only if all shards vote to commit.

\response A pre-commit transaction may abort if replication fails. As described in Section~\ref{design_decentralized}, only when replication is finished and all shards vote to commit, a transaction can be truly committed. The status of \precommit only means that all shards agree to commit the transaction, but if more than half replicas fail, the replication is failed, the transaction has to be aborted. We have underscored this point in both Fig.~\ref{transition}, Section~\ref{state transition}, and Section~\ref{recoverability}.

\vspace{3mm}

\textbf{-} What happens with the in-memory pre-commit state/data if the server reboots?

\response Rebooted server will restore committed transaction’s write data from the log. The \precommit state is a temporal state that is used to signal shard leaders for the early conclusion of \cc and has no influence on the final commit decision. Therefore, the \precommit state isn't crucial for restoration as it doesn't affect correctness.
 
\vspace{3mm}

\textbf{-}  In the evaluation, how does 2PC+2PL and 2PC+OCC work and which state-of-the-art systems do they represent ?

\response The 2PC+2PL is an implementation of Spanner's transaction protocol, and 2PC+OCC can be seen as a variant of Spanner's implementation with OCC as the concurrency control mechanism. Similar approaches have been employed by TAPIR~\cite{tapir} and Janus~\cite{janus} in their evaluations. We have clarified these in Section~\ref{setup}.


\vspace{3mm}

\textbf{-} Buffering updates on the client is briefly mentioned (line 556), but it isn't explained why this choice was made. Was this choice made also in the evaluation section for competing approaches?

\response Buffering updates on clients is a common optimization for reducing write lock duration, as seen in systems like Tapir\cite{tapir} and Carousel~\cite{carousel}. To ensure fairness, in our evaluation, all methods will buffer updates on the client during execution. 



